BEACON: Budget-Aware Entity Matching Across Domains (Extended Technical Report)

Entity Matching (EM)--the task of determining whether two data records refer to the same real-world entity--is a core task in data integration. Recent advances in deep learning have set a new standard for EM, particularly through fine-tuning Pretrained Language Models (PLMs) and, more recently, Large Language Models (LLMs). However, fine-tuning typically requires large amounts of labeled data, which are expensive and time-consuming to obtain. In the context of e-commerce matching, labeling scarcity varies widely across domains, raising the question of how to intelligently train accurate domain-specific EM models with limited labeled data. In this work we assume users have only a limited amount of labels for a specific target domain but have access to labeled data from other domains. We introduce BEACON, a distribution-aware, budget-aware framework for low-resource EM across domains. BEACON leverages the insight that embedding representations of pairwise candidate matches can guide the effective selection of out-of-domain samples under limited in-domain supervision. We conduct extensive experiments across multiple domain-partitioned datasets derived from established EM benchmarks, demonstrating that BEACON consistently outperforms state-of-the-art methods under different training budgets.

==> ablation_tables/wdc_50cc_50un_to10k_ablation.tex <==
\begin{tabular}{lccc|c}
\toprule
Method & 5.0k & 10.0k & Mean & SD \\
\midrule
SPEC & 0.710 & 0.731 & 0.697 & 0.048 \\
GEN & 0.694 & 0.729 & 0.682 & 0.064 \\
AUG & 0.693 & 0.695 & 0.681 & 0.032 \\
KCG-TV & \textbf{0.758} & \textbf{0.763} & \textbf{0.739} & 0.035 \\
KCG-TV-AUG & \underline{0.739} & \underline{0.746} & \underline{0.726} & 0.031 \\
MFSN~\cite{sun2024mfsn} & 0.681 & 0.680 & 0.668 & 0.022 \\
LLAMA~\cite{dubey2024llama} & 0.571 & 0.571 & 0.571 & 0.000 \\
JELLYFISH~\cite{zhang2023jellyfish} & 0.638 & 0.638 & 0.638 & 0.000 \\
\bottomrule
\end{tabular}

==> ablation_tables/wdc_50cc_50un_to1k_ablation.tex <==
\begin{tabular}{lccc|c}
\toprule
Method & 500 & 1.0k & Mean & SD \\
\midrule
SPEC  & 0.347 & 0.611 & 0.435 & 0.132 \\
GEN & 0.301 & 0.575 & 0.402 & 0.118 \\
AUG  & 0.379 & 0.630 & 0.432 & 0.127 \\
KCG-TV & 0.347 & \underline{0.654} & 0.443 & 0.144 \\
KCG-TV-AUG & \underline{0.437} & \textbf{0.671} & \underline{0.470} & 0.146 \\
MFSN~\cite{sun2024mfsn} & \textbf{0.577} & 0.598 & \textbf{0.541} & 0.080 \\
LLAMA~\cite{dubey2024llama} & 0.571 & 0.571 & 0.571 & 0.000 \\
JELLYFISH~\cite{zhang2023jellyfish} & 0.638 & 0.638 & 0.638 & 0.000 \\
\bottomrule
\end{tabular}

==> ablation_tables/wdc_50cc_50un_to25k_ablation.tex <==
\begin{tabular}{lccc|c}
\toprule
Method & 20.0k & 25.0k & Mean & SD \\
\midrule
SPEC & 0.724 & 0.718 & 0.721 & 0.004 \\
GEN & 0.735 & 0.740 & 0.729 & 0.013 \\
AUG & 0.699 & 0.701 & 0.699 & 0.002 \\
KCG-TV & \textbf{0.762} & \textbf{0.764} & \textbf{0.758} & 0.004 \\
KCG-TV-AUG & \underline{0.758} & \underline{0.753} & \underline{0.752} & 0.005 \\
MFSN~\cite{sun2024mfsn} & TODO & TODO & TODO & TODO \\
LLAMA~\cite{dubey2024llama} & 0.571 & 0.571 & 0.571 & 0.000 \\
JELLYFISH~\cite{zhang2023jellyfish} & 0.638 & 0.638 & 0.638 & 0.000 \\
\bottomrule
\end{tabular}
